Lighter-Than-Air Autonomous Ball Capture and Scoring Robot -- Design, Development, and Deployment

This paper describes the full end-to-end design of our primary scoring agent in an aerial autonomous robotics competition from April 2023. As open-ended robotics competitions become more popular, we wish to begin documenting successful team designs and approaches. The intended audience of this paper is not only any future or potential participant in this particular national Defend The Republic (DTR) competition, but rather anyone thinking about designing their first robot or system to be entered in a competition with clear goals. Future DTR participants can and should either build on the ideas here, or find new alternate strategies that can defeat the most successful design last time. For non-DTR participants but students interested in robotics competitions, identifying the minimum viable system needed to be competitive is still important in helping manage time and prioritizing tasks that are crucial to competition success first.

==> resources/common.tex <==
%%
%% Common commands for publication Version 0.1
%% 
%% 
%%

\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{remarks}[theorem]{Remarks}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{example}[theorem]{Example}	
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{problem}[theorem]{Problem}
\newtheorem{assumption}[theorem]{Assumption}


\newcommand{\real}{{\mathbb{R}}}
\newcommand{\realpositive}{\mathbb{R}_{>0}}
\newcommand{\realnonnegative}{\mathbb{R}_{\ge 0}}
\newcommand{\integernonnegative}{\mathbb{Z}_{\ge 0}}
\newcommand{\integerpositive}{\mathbb{Z}_{> 0}}
\newcommand{\domain}{\mathcal{D}}
\newcommand{\opendomain}{\mathcal{S}_o}
\newcommand{\closeddomain}{\mathcal{S}_c}
\newcommand{\opencurve}{\gamma_{\texttt{opc}}}
\newcommand{\closedcurve}{\gamma_{\texttt{cpc}}}
\newcommand{\dist}{\operatorname{d}}
\newcommand{\GG}{{\mathcal{G}}}
\newcommand{\PP}{{\mathcal{P}}}
\newcommand{\EE}{{\mathcal{E}}}
\newcommand{\Ac}{{\mathcal{A}}}
\newcommand{\MM}{{\mathcal{M}}}
\newcommand{\NN}{{\mathcal{N}}}
\newcommand{\LL}{{\mathcal{L}}}
\newcommand{\UU}{{\mathcal{U}}}
\renewcommand{\natural}{{\mathbb{N}}}
\newcommand{\HH}{{\mathcal{H}}}
\newcommand{\WW}{{\mathcal{W}}}
\newcommand{\data}{{\mathcal{D}}}
\newcommand{\ragents}{{\mathcal{A}}}
\newcommand{\evol}{\operatorname{Evl}}
\newcommand{\bound}{\operatorname{bnd}}
\newcommand{\halfspace}{{H}}
\newcommand{\HHc}{{\mathcal{H}}_c}
\newcommand{\HHo}{{\mathcal{H}}_o}
\newcommand{\VV}{{\mathcal{V}}}
\newcommand{\TT}{{\mathcal{T}}}
\newcommand{\CM}{{\text{CM}}}
\newcommand{\cntr}{\operatorname{cntr}}
\newcommand{\We}{{\text{We}}}
\newcommand{\cm}[1]{\operatorname{cntr}(#1)}
\newcommand{\cc}[1]{\operatorname{cc}(#1)}
\newcommand{\ccr}[1]{\operatorname{cr}(#1)}
% \newcommand{\unit}[1]{\operatorname{unit}(#1)}
\newcommand{\tbb}{\operatorname{tbb}}
\newcommand{\loc}[1]{\operatorname{loc}(#1)}
\newcommand{\normal}{\operatorname{n}}
\newcommand{\mass}[1]{\operatorname{mass}(#1)}
\newcommand{\AreaWeight}{f}
\newcommand{\ones}[1]{\mathbb{1}_{#1}}
\newcommand{\zeros}[1]{\mathbb{0}_{#1}}
\newcommand{\spn}{\operatorname{span}}
\newcommand{\diag}[1]{\operatorname{diag}\left( #1\right)}
\newcommand{\trace}[1]{\operatorname{tr}( #1)}
\newcommand{\interior}[1]{\operatorname{int}\left( #1\right)}
\renewcommand{\tilde}{\widetilde}
\newcommand{\graph}{G}
\newcommand{\vertices}{V}
\newcommand{\edges}{E}
\newcommand{\adjmat}{A}
\newcommand{\subscr}[2]{#1_{\textup{#2}}}
\newcommand{\rank}{\text{rank} \,}
\renewcommand{\div}{\text{div}}
\newcommand\reg{$^{\textrm{\tiny\textregistered}}$\xspace}
\newcommand{\Polygon}{\mathcal{P}}
\newcommand{\proj}{\operatorname{pr}}
\newcommand{\automaton}{\texttt{intersection-free gradient automaton}}
\newcommand{\vmax}{v_{\text{max}}}
\newcommand{\timestep}{\Delta t}
\newcommand{\sleep}{t_\text{sleep}}
\newcommand{\goal}{p_\text{goal}}
\newcommand{\eps}{\varepsilon}
\renewcommand{\epsilon}{\varepsilon}
\newcommand{\diam}{\operatorname{diam}}
\DeclareMathOperator*{\argmin}{\operatorname{arg\,min}}

\newcommand{\gV}{\text{g}V}
\newcommand{\ghV}{\text{g}\hat{V}}
\newcommand{\dgV}{\text{dg}V}
\newcommand{\dghV}{\text{dg}\hat{V}}
\newcommand{\gVV}{\text{g}\mathcal{V}}
\newcommand{\dgVV}{\text{dg}\mathcal{V}}
\newcommand{\gN}{\text{g}\NN}
\newcommand{\dgN}{\text{dg}\NN}

\newcommand{\algostep}[1]{{\small\texttt{#1:}}\xspace}
\newcommand{\CVT}{\operatorname{CVT}}

\newcommand{\Algo}{\operatorname{T}}
\newcommand{\CentroidPowerAlgo}{\operatorname{T_{quad-perf}}}
\newcommand{\WeberWeightedAlgo}{\operatorname{T_{linear-perf}}}

\newcommand{\outside}{\textup{out}}
\newcommand{\inside}{\textup{in}}
\newcommand{\Outside}{\textup{Outside}}
\newcommand{\Inside}{\textup{Inside}}
\newcommand{\versor}{\textup{unit}}
\newcommand{\until}[1]{\{1,\dots, #1\}}
\newcommand{\fromto}[2]{\langle #1,\dots, #2 \rangle}
\newcommand{\sgn}[1]{\operatorname{sgn}(#1)}
\newcommand{\map}[3]{#1: #2 \rightarrow #3}
\newcommand{\svmap}[3]{#1: #2 \rightrightarrows #3}
\newcommand{\setdef}[2]{\{#1 \; | \; #2\}}
\newcommand{\pder}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\ppder}[2]{\frac{\partial^2 #1}{\partial #2^2}}
\newcommand{\pcder}[3]{\frac{\partial^2 #1}{\partial #2 \partial #3}}
\newcommand{\oball}[2]{B(#1,#2)}
\newcommand{\cball}[2]{\overline{B}(#1,#2)}
\newcommand{\inn}[2]{\langle #1,#2 \rangle}
\newcommand{\osegment}[2]{]#1,#2[}
\newcommand{\csegment}[2]{[#1,#2]}
\newcommand{\cosegment}[2]{[#1,#2[}
\newcommand{\ray}[2]{\texttt{ray}(#1,#2)}
\renewcommand{\wedge}[3]{\texttt{wedge}(#1,#2,#3)}
\newcommand{\TwoNorm}[1]{\|#1\|}
\newcommand{\ortho}[1]{#1^\perp}
\newcommand{\variance}[1]{\operatorname{var}(#1)}
\renewcommand{\hat}{\widehat}

\newcommand{\algoMotionControl}{\texttt{motion control law}\xspace}
\newcommand{\algoOneStep}{\texttt{one-step-ahead update policy}\xspace}
\newcommand{\algoMultiStep}{\texttt{multiple-steps-ahead update  policy}\xspace}
\newcommand{\algoVoronoi}{\texttt{Voronoi cell computation}\xspace}
\newcommand{\algoFull}{\texttt{self-triggered centroid
    algorithm}\xspace}
\newcommand{\falgoFull}{f_{\operatorname{stca}}}
\newcommand{\fmotion}{f_{\operatorname{motion}}}
\newcommand{\finfo}{f_{\operatorname{info}}}

\newcommand{\oprocendsymbol}{\hbox{$\bullet$}}
\newcommand{\oprocend}{\relax\ifmmode\else\unskip\hfill\fi\oprocendsymbol}
\def\eqoprocend{\tag*{$\bullet$}}

% this wraps theorem titles (or proposition, etc)
\newcommand{\longthmtitle}[1]{\mbox{}\textup{\textbf{(#1)}}}

%% Enumerate environment
\renewcommand{\theenumi}{(\roman{enumi})}
\renewcommand{\labelenumi}{\theenumi}

\newcommand{\margin}[1]{\marginpar{\color{red}\tiny\ttfamily#1}}
\newcommand{\todo}[1]{\par\noindent{\color{blue}
    \raggedright\textsc{#1}\par\marginpar{\Large $\star$}}}

\newcommand{\myclearpage}{\clearpage}
\renewcommand{\myclearpage}{}

\renewcommand{\cm}[1]{C_{#1}}
\renewcommand{\mass}[1]{M_{#1}}

\newcommand{\comment}[1]{}

%
\definecolor{ashgrey}{rgb}{0.7, 0.75, 0.71}
